METAFOR: A Hybrid Metaheuristics Software Framework for Single-Objective Continuous Optimization Problems

Hybrid metaheuristics are powerful techniques for solving difficult optimization problems that exploit the strengths of different approaches in a single implementation. For algorithm designers, however, creating hybrid metaheuristic implementations has become increasingly challenging due to the vast number of design options available in the literature and the fact that they often rely on their knowledge and intuition to come up with new algorithm designs. In this paper, we propose a modular metaheuristic software framework, called METAFOR, that can be coupled with an automatic algorithm configuration tool to automatically design hybrid metaheuristics. METAFOR is specifically designed to hybridize Particle Swarm Optimization, Differential Evolution and Covariance Matrix Adaptation-Evolution Strategy, and includes a local search module that allows their execution to be interleaved with a subordinate local search. We use the configuration tool irace to automatically generate 17 different metaheuristic implementations and evaluate their performance on a diverse set of continuous optimization problems. Our results show that, across all the considered problem classes, automatically generated hybrid implementations are able to outperform configured single-approach implementations, while these latter offer advantages on specific classes of functions. We provide useful insights on the type of hybridization that works best for specific problem classes, the algorithm components that contribute to the performance of the algorithms, and the advantages and disadvantages of two well-known instance separation strategies, creating stratified training set using a fix percentage and leave-one-class-out cross-validation.

==> tables/tbl_LD_1.tex <==
\begin{ThreePartTable}
\setlength{\tabcolsep}{0.5pt} % Default value: 6pt
    {\fontsize{6.5}{6.2}\selectfont
    \begin{longtable}{m{0.1cm} C{1.25cm} m{0.88cm} m{0.88cm} m{0.88cm} m{0.88cm} m{0.88cm} m{0.88cm} m{0.88cm} m{0.88cm} m{0.88cm} m{0.88cm} m{0.88cm} m{0.88cm} m{0.88cm} m{0.88cm}} %{@{} c | *{10}{c} @{}} %{ l c c c c c c c c c c c c c c c c}
    \caption{Average median (Av.MED), average median error (Av.MEDerr) and average median absolute deviation (Av.MAD) obtained by the algorithms on the 19 functions of the SOCO'10 test suite with $\mathbf{d = 500}$.}\label{table:MED-MEDerr-MAD-LD-500}\\
    \toprule
    & $f\#$ &  
    %&  & 
    \textbf{\MTFtfoTBL} &  \textbf{\MTFldoTBL} & 
    \textbf{\CMAEStfoTBL} & \textbf{\CMAESldoTBL} & 
    \textbf{\DEtfoTBL} & \textbf{\DEldoTBL} & 
    \textbf{\PSOtfoTBL} & \textbf{\PSOldoTBL} & 
    \textbf{\PDHybtfoTBL} & \textbf{\PDHybldoTBL} & 
    \textbf{\DCHybtfoTBL} & \textbf{\DCHybldoTBL} &
    \textbf{\PCHybtfoTBL} & \textbf{\PCHybldoTBL} \\
    \midrule
    \endfirsthead
    
    \caption*{ Table \ref{table:MED-MEDerr-MAD-LD-500} (Continued.)}\\
    \toprule
    & $f\#$ &  
    %&  & 
    \textbf{\MTFtfoTBL} &  \textbf{\MTFldoTBL} & 
    \textbf{\CMAEStfoTBL} & \textbf{\CMAESldoTBL} & 
    \textbf{\DEtfoTBL} & \textbf{\DEldoTBL} & 
    \textbf{\PSOtfoTBL} & \textbf{\PSOldoTBL} & 
    \textbf{\PDHybtfoTBL} & \textbf{\PDHybldoTBL} & 
    \textbf{\DCHybtfoTBL} & \textbf{\DCHybldoTBL} &
    \textbf{\PCHybtfoTBL} & \textbf{\PCHybldoTBL} \\
    \midrule
    \endhead
    
    \bottomrule
    %\insertTableNotes
    \endfoot
    
    \bottomrule
    %\insertTableNotes  % tell LaTeX where to insert the contents of "TableNotes"
    \endlastfoot

%%%%%%% Values here
%%%%% MED %%%%%
% \multirow{18}{*}{\rotatebox[origin=c]{90}{MEDIAN SOLUTION}} & $f_{1} (d=500)$ & 	5.34e-21 & 	9.81e-20 & 	1.39e-16 & 	2.01e-22 & 	\textbf{0.00e+00} & 	2.79e-03 & 	5.63e-14 & 	4.93e+04 & 	4.56e-26 & 	9.93e-22 & 	3.31e-20 & 	2.32e-22 & 	8.18e-22 & 	1.28e-21 \\
% & $f_{5} (d=500)$ & 	1.18e+01 & 	1.24e+01 & 	\textbf{8.92e-01} & 	1.16e+01 & 	1.30e+02 & 	1.30e+02 & 	1.02e+02 & 	8.63e+01 & 	7.43e+01 & 	1.36e+02 & 	1.10e+01 & 	1.69e+01 & 	1.32e+01 & 	6.10e+00 \\
% & $f_{6} (d=500)$ & 	1.79e+05 & 	1.85e+05 & 	1.61e+05 & 	1.69e+05 & 	1.18e+06 & 	6.76e+05 & 	\textbf{3.56e+04} & 	5.14e+05 & 	1.31e+05 & 	6.73e+05 & 	1.90e+05 & 	2.08e+05 & 	1.99e+05 & 	1.73e+05 \\
% & $f_{8} (d=500)$ & 	1.00e+10 & 	\textbf{0.00e+00} & 	4.45e-12 & 	4.08e-12 & 	\textbf{0.00e+00} & 	2.06e-02 & 	1.45e+03 & 	1.98e+03 & 	4.44e-16 & 	\textbf{0.00e+00} & 	6.63e-12 & 	5.65e-12 & 	1.00e+10 & 	1.00e+10 \\
% & $f_{9} (d=500)$ & 	1.36e+00 & 	1.09e+00 & 	3.02e+00 & 	1.95e+00 & 	\textbf{9.03e-02} & 	3.61e+02 & 	3.34e+03 & 	3.97e+03 & 	4.45e+01 & 	1.60e+00 & 	8.29e-01 & 	9.25e-01 & 	7.82e-01 & 	1.37e+00 \\
% & $f_{10} (d=500)$ & 	1.49e+00 & 	1.24e-18 & 	5.25e+00 & 	3.15e+00 & 	\textbf{0.00e+00} & 	1.85e-02 & 	3.11e+02 & 	1.02e+04 & 	8.40e+00 & 	1.32e-25 & 	4.41e-01 & 	1.05e+00 & 	7.50e-22 & 	2.10e+00 \\
% & $f_{13} (d=500)$ & 	4.05e-13 & 	1.44e-16 & 	2.23e-13 & 	1.95e-13 & 	\textbf{1.30e-16} & 	3.19e-01 & 	1.94e+01 & 	2.04e+01 & 	3.08e-11 & 	1.18e-13 & 	5.33e-13 & 	4.67e-13 & 	7.41e-13 & 	4.39e-13 \\
% & $f_{15} (d=500)$ & 	\textbf{4.74e+02} & 	4.75e+02 & 	4.75e+02 & 	\textbf{4.74e+02} & 	7.27e+02 & 	8.38e+03 & 	6.53e+02 & 	1.00e+10 & 	4.75e+02 & 	1.00e+03 & 	4.77e+02 & 	4.75e+02 & 	4.78e+02 & 	4.75e+02 \\
% & $f_{17} (d=500)$ & 	1.63e-19 & 	3.79e-19 & 	6.73e-17 & 	1.63e-19 & 	8.94e-19 & 	6.94e-03 & 	5.09e-07 & 	2.68e+03 & 	8.13e-19 & 	2.00e-04 & 	1.63e-19 & 	1.63e-19 & 	\textbf{1.08e-19} & 	1.63e-19 \\
% & $f_{19} (d=500)$ & 	2.98e+02 & 	4.34e+02 & 	4.06e+02 & 	3.32e+02 & 	1.98e+02 & 	3.37e+02 & 	1.64e+04 & 	5.59e+04 & 	5.76e+02 & 	\textbf{7.52e+00} & 	2.71e+02 & 	4.42e+02 & 	2.31e+02 & 	3.41e+02 \\
% & $f_{21} (d=500)$ & 	2.43e+05 & 	2.42e+05 & 	2.57e+05 & 	2.49e+05 & 	2.19e+05 & 	2.19e+05 & 	3.14e+05 & 	3.56e+05 & 	2.48e+05 & 	\textbf{2.13e+05} & 	2.41e+05 & 	2.41e+05 & 	2.40e+05 & 	2.44e+05 \\
% & $f_{27} (d=500)$ & 	8.70e+02 & 	8.36e+02 & 	8.41e+02 & 	9.14e+02 & 	\textbf{6.69e-08} & 	4.39e+01 & 	1.11e+03 & 	1.59e+05 & 	1.04e+02 & 	2.10e-02 & 	6.44e+02 & 	8.26e+02 & 	5.35e+02 & 	7.73e+02 \\
% & $f_{28} (d=500)$ & 	1.29e+03 & 	1.25e+03 & 	1.27e+03 & 	1.34e+03 & 	\textbf{4.19e+02} & 	8.21e+03 & 	2.12e+03 & 	1.00e+10 & 	4.96e+02 & 	6.49e+02 & 	1.18e+03 & 	1.27e+03 & 	1.17e+03 & 	1.23e+03 \\
% & $f_{29} (d=500)$ & 	5.22e+02 & 	4.21e+01 & 	4.61e+02 & 	6.07e+02 & 	8.32e+01 & 	1.48e+02 & 	3.59e+03 & 	4.65e+03 & 	4.18e+02 & 	\textbf{1.28e+01} & 	3.43e+02 & 	4.32e+02 & 	3.25e+02 & 	3.95e+02 \\
% & $f_{30} (d=500)$ & 	1.87e-08 & 	3.18e-09 & 	7.47e-08 & 	7.61e-07 & 	\textbf{5.54e-32} & 	4.40e-02 & 	7.17e+03 & 	1.01e+04 & 	4.20e+00 & 	4.93e-25 & 	2.54e-11 & 	3.88e-09 & 	1.44e-11 & 	1.32e-09 \\
% & $f_{31} (d=500)$ & 	1.67e+03 & 	1.60e+03 & 	1.58e+03 & 	1.81e+03 & 	\textbf{1.50e-05} & 	1.27e+02 & 	2.22e+03 & 	4.73e+04 & 	1.42e+02 & 	1.15e-02 & 	6.27e+02 & 	1.61e+03 & 	1.55e+02 & 	1.47e+03 \\
% & $f_{32} (d=500)$ & 	2.96e+03 & 	2.87e+03 & 	2.94e+03 & 	3.11e+03 & 	\textbf{8.39e+01} & 	1.51e+03 & 	3.51e+03 & 	3.61e+03 & 	3.95e+02 & 	1.48e+02 & 	2.54e+03 & 	2.89e+03 & 	2.36e+03 & 	2.77e+03 \\
% & $f_{33} (d=500)$ & 	4.80e+02 & 	3.87e+02 & 	3.62e+02 & 	5.82e+02 & 	1.10e+01 & 	5.60e+01 & 	1.65e+03 & 	1.14e+03 & 	1.71e+02 & 	\textbf{2.93e+00} & 	7.73e+01 & 	4.43e+02 & 	7.48e+01 & 	2.86e+02 \\
% & $f_{34} (d=500)$ & 	6.30e+00 & 	3.15e+00 & 	2.10e+00 & 	1.15e+01 & 	9.49e-20 & 	1.05e+00 & 	1.86e+04 & 	2.66e+04 & 	9.45e+00 & 	\textbf{6.91e-30} & 	1.13e-12 & 	5.25e+00 & 	1.43e-12 & 	1.05e+00 \\
& {Wins \newline (MED) } & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{10} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{6} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{0} \\
%MTF.25OUT & MTF.LDO & CMAES.25OUT & CMAES.LDO & DE.25OUT & DE.LDO & PSO.X.25OUT & PSO.X.LDO & PSO.DE.25OUT & PSO.DE.LDO & DE.CMAES.25OUT & DE.CMAES.LDO & PSO.CMAES.25OUT & PSO.CMAES.LDO \\
\midrule
%Functions  1  -  7 \\
\multirow{2}{*}{\rotatebox[origin=c]{90}{SHU}} & Av.MED  & 1.43e+09 & 2.64e+04 & 2.30e+04 & 2.41e+04 & 1.69e+05 & 9.66e+04 & \textbf{5.83e+03} & 8.28e+04 & 1.87e+04 & 9.62e+04 & 2.71e+04 & 2.97e+04 & 1.43e+09 & 1.43e+09 \\
& Av.Ranking  & 7.57 & 5.29 & 6.71 & 5.57 & \textbf{4.86} & 11.00 & 10.43 & 12.57 & 7.29 & 6.86 & 6.57 & 6.86 & 7.14 & 7.29 \\
\midrule
%Functions  8  -  11 \\
\multirow{2}{*}{\rotatebox[origin=c]{90}{MUL}} & Av.MED  & 4.88e+04 & 4.86e+04 & 5.16e+04 & 5.00e+04 & 4.40e+04 & 4.55e+04 & 6.62e+04 & 2.00e+09 & 4.98e+04 & \textbf{4.28e+04} & 4.83e+04 & 4.84e+04 & 4.81e+04 & 4.90e+04 \\
& Av.Ranking  & 8.55 & 7.36 & 9.27 & 9.64 & \textbf{3.18} & 7.00 & 12.55 & 13.91 & 6.91 & 3.55 & 5.64 & 8.36 & 4.36 & 6.91 \\
\midrule
%Functions  12  -  19 \\
\multirow{2}{*}{\rotatebox[origin=c]{90}{HYB}} & Av.MED  & 2.79e+04 & 2.77e+04 & 2.94e+04 & 2.86e+04 & 2.44e+04 & 2.55e+04 & 3.93e+04 & 1.11e+09 & 2.77e+04 & \textbf{2.38e+04} & 2.74e+04 & 2.76e+04 & 2.72e+04 & 2.79e+04 \\
& Av.Ranking  & 4.95 & 4.21 & 5.47 & 7.21 & \textbf{3.53} & 5.95 & 9.53 & 10.47 & 7.84 & 6.53 & 8.53 & 10.68 & 9.37 & 10.84 \\
\midrule
%Functions  1  -  19 \\
\multirow{2}{*}{\rotatebox[origin=c]{90}{ALL}} & Av.MED  & 5.26e+08 & 2.29e+04 & 2.24e+04 & 2.25e+04 & 7.37e+04 & 4.81e+04 & 2.17e+04 & 1.05e+09 & \textbf{2.01e+04} & 4.67e+04 & 2.30e+04 & 2.41e+04 & 5.26e+08 & 5.26e+08 \\
& Av.Ranking  & 8.26 & 6.63 & 8.21 & 8.26 & \textbf{3.74} & 8.42 & 11.79 & 13.42 & 7.26 & 4.63 & 5.84 & 7.84 & 5.37 & 7.00 \\
\midrule
%Best algorithm across all functions: DE.25OUT	
%DE.25OUT 1 1 1 1 NA 0.475293349555944 0.677797900477078 0.216515418578437 1 1 1 1 1 1
& \multicolumn{1}{c}{Wilcoxon test} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} \\

%%%%% MEDerr %%%%%
\toprule
% \multirow{18}{*}{\rotatebox[origin=c]{90}{MEDIAN SOLUTION ERROR}} & $f_{1} (d=500)$ & 	5.34e-21 & 	9.81e-20 & 	1.39e-16 & 	2.01e-22 & 	\textbf{0.00e+00} & 	2.79e-03 & 	5.63e-14 & 	4.93e+04 & 	4.56e-26 & 	9.93e-22 & 	3.31e-20 & 	2.32e-22 & 	8.18e-22 & 	1.28e-21 \\
% & $f_{5} (d=500)$ & 	1.16e+01 & 	1.22e+01 & 	\textbf{6.68e-01} & 	1.14e+01 & 	1.30e+02 & 	1.30e+02 & 	1.02e+02 & 	8.61e+01 & 	7.41e+01 & 	1.36e+02 & 	1.08e+01 & 	1.67e+01 & 	1.30e+01 & 	5.88e+00 \\
% & $f_{6} (d=500)$ & 	1.57e+05 & 	1.63e+05 & 	1.39e+05 & 	1.47e+05 & 	1.16e+06 & 	6.54e+05 & 	\textbf{1.40e+04} & 	4.92e+05 & 	1.09e+05 & 	6.51e+05 & 	1.68e+05 & 	1.86e+05 & 	1.77e+05 & 	1.51e+05 \\
% & $f_{8} (d=500)$ & 	1.00e+10 & 	\textbf{0.00e+00} & 	4.45e-12 & 	4.08e-12 & 	\textbf{0.00e+00} & 	2.06e-02 & 	1.45e+03 & 	1.98e+03 & 	4.44e-16 & 	\textbf{0.00e+00} & 	6.63e-12 & 	5.65e-12 & 	1.00e+10 & 	1.00e+10 \\
% & $f_{9} (d=500)$ & 	1.29e+00 & 	1.02e+00 & 	2.95e+00 & 	1.88e+00 & 	\textbf{2.31e-02} & 	3.61e+02 & 	3.34e+03 & 	3.97e+03 & 	4.44e+01 & 	1.53e+00 & 	7.62e-01 & 	8.58e-01 & 	7.15e-01 & 	1.30e+00 \\
% & $f_{10} (d=500)$ & 	1.49e+00 & 	1.24e-18 & 	5.25e+00 & 	3.15e+00 & 	\textbf{0.00e+00} & 	1.85e-02 & 	3.11e+02 & 	1.02e+04 & 	8.40e+00 & 	1.32e-25 & 	4.41e-01 & 	1.05e+00 & 	7.50e-22 & 	2.10e+00 \\
% & $f_{13} (d=500)$ & 	4.05e-13 & 	1.28e-16 & 	2.23e-13 & 	1.95e-13 & 	\textbf{1.14e-16} & 	3.19e-01 & 	1.94e+01 & 	2.04e+01 & 	3.08e-11 & 	1.18e-13 & 	5.33e-13 & 	4.67e-13 & 	7.41e-13 & 	4.39e-13 \\
% & $f_{15} (d=500)$ & 	\textbf{1.52e+02} & 	1.53e+02 & 	1.53e+02 & 	\textbf{1.52e+02} & 	4.05e+02 & 	8.06e+03 & 	3.31e+02 & 	1.00e+10 & 	1.53e+02 & 	6.78e+02 & 	1.55e+02 & 	1.53e+02 & 	1.56e+02 & 	1.53e+02 \\
% & $f_{17} (d=500)$ & 	5.46e-20 & 	2.71e-19 & 	6.72e-17 & 	5.46e-20 & 	7.86e-19 & 	6.94e-03 & 	5.09e-07 & 	2.68e+03 & 	7.05e-19 & 	2.00e-04 & 	5.46e-20 & 	5.46e-20 & 	\textbf{4.20e-22} & 	5.46e-20 \\
% & $f_{19} (d=500)$ & 	2.98e+02 & 	4.34e+02 & 	4.06e+02 & 	3.32e+02 & 	1.98e+02 & 	3.37e+02 & 	1.64e+04 & 	5.59e+04 & 	5.76e+02 & 	\textbf{7.52e+00} & 	2.71e+02 & 	4.42e+02 & 	2.31e+02 & 	3.41e+02 \\
% & $f_{21} (d=500)$ & 	3.08e+04 & 	2.98e+04 & 	4.48e+04 & 	3.68e+04 & 	6.75e+03 & 	6.75e+03 & 	1.02e+05 & 	1.44e+05 & 	3.58e+04 & 	\textbf{7.54e+02} & 	2.88e+04 & 	2.88e+04 & 	2.78e+04 & 	3.18e+04 \\
% & $f_{27} (d=500)$ & 	8.70e+02 & 	8.36e+02 & 	8.41e+02 & 	9.14e+02 & 	\textbf{6.60e-08} & 	4.39e+01 & 	1.11e+03 & 	1.59e+05 & 	1.04e+02 & 	2.10e-02 & 	6.44e+02 & 	8.26e+02 & 	5.35e+02 & 	7.73e+02 \\
% & $f_{28} (d=500)$ & 	1.09e+03 & 	1.05e+03 & 	1.07e+03 & 	1.14e+03 & 	\textbf{2.18e+02} & 	8.01e+03 & 	1.92e+03 & 	1.00e+10 & 	2.95e+02 & 	4.48e+02 & 	9.79e+02 & 	1.07e+03 & 	9.69e+02 & 	1.03e+03 \\
% & $f_{29} (d=500)$ & 	5.21e+02 & 	4.10e+01 & 	4.60e+02 & 	6.06e+02 & 	8.21e+01 & 	1.47e+02 & 	3.59e+03 & 	4.65e+03 & 	4.17e+02 & 	\textbf{1.17e+01} & 	3.42e+02 & 	4.31e+02 & 	3.24e+02 & 	3.94e+02 \\
% & $f_{30} (d=500)$ & 	1.87e-08 & 	3.18e-09 & 	7.47e-08 & 	7.61e-07 & 	\textbf{5.54e-32} & 	4.40e-02 & 	7.17e+03 & 	1.01e+04 & 	4.20e+00 & 	4.93e-25 & 	2.54e-11 & 	3.88e-09 & 	1.44e-11 & 	1.32e-09 \\
% & $f_{31} (d=500)$ & 	1.67e+03 & 	1.60e+03 & 	1.58e+03 & 	1.81e+03 & 	\textbf{1.50e-05} & 	1.27e+02 & 	2.22e+03 & 	4.73e+04 & 	1.42e+02 & 	1.15e-02 & 	6.27e+02 & 	1.61e+03 & 	1.55e+02 & 	1.47e+03 \\
% & $f_{32} (d=500)$ & 	2.94e+03 & 	2.85e+03 & 	2.92e+03 & 	3.09e+03 & 	\textbf{6.75e+01} & 	1.49e+03 & 	3.49e+03 & 	3.59e+03 & 	3.79e+02 & 	1.32e+02 & 	2.52e+03 & 	2.87e+03 & 	2.34e+03 & 	2.75e+03 \\
% & $f_{33} (d=500)$ & 	4.80e+02 & 	3.87e+02 & 	3.62e+02 & 	5.82e+02 & 	1.10e+01 & 	5.60e+01 & 	1.65e+03 & 	1.14e+03 & 	1.71e+02 & 	\textbf{2.93e+00} & 	7.73e+01 & 	4.43e+02 & 	7.48e+01 & 	2.86e+02 \\
% & $f_{34} (d=500)$ & 	6.30e+00 & 	3.15e+00 & 	2.10e+00 & 	1.15e+01 & 	9.49e-20 & 	1.05e+00 & 	1.86e+04 & 	2.66e+04 & 	9.45e+00 & 	\textbf{6.91e-30} & 	1.13e-12 & 	5.25e+00 & 	1.43e-12 & 	1.05e+00 \\
& {Wins \newline (MEDerr) } & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{10} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{6} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{0} \\
%MTF.25OUT & MTF.LDO & CMAES.25OUT & CMAES.LDO & DE.25OUT & DE.LDO & PSO.X.25OUT & PSO.X.LDO & PSO.DE.25OUT & PSO.DE.LDO & DE.CMAES.25OUT & DE.CMAES.LDO & PSO.CMAES.25OUT & PSO.CMAES.LDO \\
\midrule
%Functions  1  -  7 \\
\multirow{2}{*}{\rotatebox[origin=c]{90}{SHU}} & Av.MEDerr  & 1.43e+09 & 2.33e+04 & 1.99e+04 & 2.10e+04 & 1.66e+05 & 9.35e+04 & \textbf{2.75e+03} & 7.97e+04 & 1.56e+04 & 9.30e+04 & 2.40e+04 & 2.66e+04 & 1.43e+09 & 1.43e+09 \\
& Av.Ranking  & 7.57 & 5.29 & 6.71 & 5.57 & \textbf{4.86} & 11.00 & 10.43 & 12.57 & 7.29 & 6.86 & 6.57 & 6.86 & 7.14 & 7.29 \\
\midrule
%Functions  8  -  11 \\
\multirow{2}{*}{\rotatebox[origin=c]{90}{MUL}} & Av.MEDerr  & 6.25e+03 & 6.08e+03 & 9.07e+03 & 7.46e+03 & 1.47e+03 & 3.03e+03 & 2.38e+04 & 2.00e+09 & 7.31e+03 & \textbf{2.88e+02} & 5.85e+03 & 5.88e+03 & 5.64e+03 & 6.46e+03 \\
& Av.Ranking  & 8.55 & 7.36 & 9.27 & 9.64 & \textbf{3.18} & 7.00 & 12.55 & 13.91 & 6.91 & 3.55 & 5.64 & 8.36 & 4.36 & 6.91 \\
\midrule
%Functions  12  -  19 \\
\multirow{2}{*}{\rotatebox[origin=c]{90}{HYB}} & Av.MEDerr  & 4.26e+03 & 4.06e+03 & 5.78e+03 & 4.99e+03 & 7.92e+02 & 1.85e+03 & 1.58e+04 & 1.11e+09 & 4.15e+03 & \textbf{1.50e+02} & 3.78e+03 & 4.01e+03 & 3.58e+03 & 4.28e+03 \\
& Av.Ranking  & 4.95 & 4.21 & 5.47 & 7.21 & \textbf{3.53} & 5.95 & 9.53 & 10.47 & 7.84 & 6.53 & 8.53 & 10.68 & 9.37 & 10.84 \\
\midrule
%Functions  1  -  19 \\
\multirow{2}{*}{\rotatebox[origin=c]{90}{ALL}} & Av.MEDerr  & 5.26e+08 & 1.05e+04 & 1.01e+04 & 1.01e+04 & 6.15e+04 & 3.58e+04 & 9.35e+03 & 1.05e+09 & \textbf{7.75e+03} & 3.44e+04 & 1.07e+04 & 1.17e+04 & 5.26e+08 & 5.26e+08 \\
& Av.Ranking  & 8.26 & 6.63 & 8.21 & 8.26 & \textbf{3.74} & 8.42 & 11.79 & 13.42 & 7.26 & 4.63 & 5.84 & 7.84 & 5.37 & 7.00 \\
\midrule
%Best algorithm across all functions: DE.25OUT	
%DE.25OUT 1 1 1 1 NA 0.475293349555944 0.677797900477078 0.216515418578437 1 1 1 1 1 1
& \multicolumn{1}{c}{Wilcoxon test} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} \\

%%%%% MAD %%%%%
\toprule
% \multirow{18}{*}{\rotatebox[origin=c]{90}{MEDIAN ABSOLUTE DEVIATION}} & $f_{1} (d=500)$ & 	3.47e-22 & 	1.87e-21 & 	5.00e-18 & 	2.61e-23 & 	\textbf{0.00e+00} & 	2.01e-03 & 	2.08e-13 & 	1.31e+04 & 	2.05e-26 & 	9.79e-22 & 	3.42e-21 & 	2.92e-23 & 	3.38e-23 & 	1.87e-23 \\
% & $f_{5} (d=500)$ & 	2.36e+00 & 	3.05e+00 & 	\textbf{4.34e-01} & 	2.00e+00 & 	4.13e+00 & 	4.79e+00 & 	1.64e+00 & 	1.39e+00 & 	3.22e+00 & 	1.45e+00 & 	1.29e+00 & 	1.36e+00 & 	2.97e+00 & 	2.69e+00 \\
% & $f_{6} (d=500)$ & 	\textbf{1.92e+03} & 	1.13e+04 & 	1.71e+04 & 	1.46e+04 & 	1.39e+05 & 	3.89e+04 & 	4.34e+03 & 	3.48e+04 & 	3.91e+03 & 	4.49e+04 & 	3.01e+04 & 	1.39e+04 & 	1.51e+04 & 	1.69e+04 \\
% & $f_{8} (d=500)$ & 	\textbf{0.00e+00} & 	\textbf{0.00e+00} & 	1.96e-14 & 	2.37e-13 & 	\textbf{0.00e+00} & 	1.97e-03 & 	3.96e+01 & 	2.20e+02 & 	4.44e-16 & 	\textbf{0.00e+00} & 	3.93e-14 & 	2.49e-13 & 	\textbf{0.00e+00} & 	\textbf{0.00e+00} \\
% & $f_{9} (d=500)$ & 	2.74e-02 & 	\textbf{1.68e-02} & 	3.09e-01 & 	2.77e-01 & 	2.30e-02 & 	2.52e+01 & 	1.70e+01 & 	3.64e+01 & 	2.90e+00 & 	3.82e-02 & 	2.21e-01 & 	2.19e-01 & 	3.04e-01 & 	3.35e-01 \\
% & $f_{10} (d=500)$ & 	2.97e-02 & 	3.62e-20 & 	8.16e-01 & 	6.48e-04 & 	\textbf{0.00e+00} & 	1.94e-03 & 	2.28e+01 & 	2.65e+02 & 	2.10e+00 & 	2.07e-26 & 	4.41e-01 & 	1.30e+01 & 	2.61e-23 & 	2.10e+00 \\
% & $f_{13} (d=500)$ & 	1.35e-15 & 	\textbf{1.80e-20} & 	3.71e-15 & 	4.68e-15 & 	1.11e-15 & 	2.85e-01 & 	3.19e-02 & 	3.03e-02 & 	2.60e-11 & 	3.76e-14 & 	2.55e-15 & 	3.16e-15 & 	2.19e-14 & 	2.36e-15 \\
% & $f_{15} (d=500)$ & 	1.57e+00 & 	2.40e-01 & 	1.75e-01 & 	1.45e+00 & 	2.35e+02 & 	1.68e+03 & 	2.88e+02 & 	\textbf{0.00e+00} & 	3.58e+00 & 	1.50e+02 & 	2.05e+00 & 	4.59e+00 & 	1.71e-02 & 	2.13e+00 \\
% & $f_{17} (d=500)$ & 	\textbf{3.70e-22} & 	4.71e-22 & 	3.93e-18 & 	\textbf{3.70e-22} & 	2.76e-20 & 	2.51e-03 & 	4.03e-07 & 	1.70e+02 & 	5.41e-20 & 	2.00e-04 & 	\textbf{3.70e-22} & 	\textbf{3.70e-22} & 	4.20e-22 & 	\textbf{3.70e-22} \\
% & $f_{19} (d=500)$ & 	2.34e+01 & 	1.03e+02 & 	2.03e+01 & 	2.84e+01 & 	1.94e+01 & 	3.32e+01 & 	1.76e+03 & 	3.93e+03 & 	1.23e+01 & 	2.22e+00 & 	3.36e+00 & 	2.06e+02 & 	\textbf{2.16e+00} & 	2.21e+01 \\
% & $f_{21} (d=500)$ & 	2.32e+03 & 	2.79e+03 & 	3.10e+03 & 	2.45e+03 & 	1.31e+03 & 	\textbf{3.36e+02} & 	2.32e+04 & 	1.88e+03 & 	2.42e+03 & 	3.39e+02 & 	2.32e+03 & 	2.00e+03 & 	2.73e+03 & 	2.41e+03 \\
% & $f_{27} (d=500)$ & 	2.99e+01 & 	3.15e+01 & 	3.21e+01 & 	2.70e+01 & 	\textbf{2.45e-06} & 	2.75e+00 & 	3.13e+01 & 	1.89e+04 & 	3.16e+01 & 	2.10e-02 & 	3.62e+01 & 	1.31e+02 & 	4.14e+01 & 	1.89e+01 \\
% & $f_{28} (d=500)$ & 	3.53e+01 & 	3.10e+01 & 	3.49e+01 & 	2.04e+01 & 	2.24e+02 & 	2.84e+03 & 	3.96e+02 & 	\textbf{0.00e+00} & 	2.63e+01 & 	2.21e+02 & 	3.26e+01 & 	1.96e+01 & 	2.17e+01 & 	1.44e+01 \\
% & $f_{29} (d=500)$ & 	9.57e+00 & 	3.26e+02 & 	3.32e+01 & 	1.29e+02 & 	1.72e+01 & 	2.53e+01 & 	3.10e+02 & 	2.23e+02 & 	2.75e+01 & 	\textbf{3.53e+00} & 	1.30e+01 & 	6.92e+01 & 	3.06e+01 & 	2.86e+01 \\
% & $f_{30} (d=500)$ & 	1.59e-08 & 	2.00e-09 & 	3.54e-08 & 	1.57e+00 & 	\textbf{5.42e-32} & 	3.98e-03 & 	3.26e+02 & 	3.12e+00 & 	2.10e+00 & 	1.71e-25 & 	2.57e-11 & 	2.34e-09 & 	1.47e-12 & 	4.73e-10 \\
% & $f_{31} (d=500)$ & 	4.48e+01 & 	2.18e+01 & 	3.83e+01 & 	3.45e+01 & 	\textbf{7.93e-03} & 	5.78e+01 & 	1.49e+01 & 	4.53e+04 & 	4.45e+01 & 	6.20e-02 & 	3.63e+02 & 	1.86e+01 & 	3.24e+01 & 	3.85e+01 \\
% & $f_{32} (d=500)$ & 	4.61e+01 & 	3.69e+01 & 	2.24e+01 & 	\textbf{1.98e+01} & 	3.34e+01 & 	4.50e+02 & 	3.00e+02 & 	1.52e+02 & 	1.52e+02 & 	3.52e+01 & 	3.75e+01 & 	1.99e+01 & 	4.36e+01 & 	2.83e+01 \\
% & $f_{33} (d=500)$ & 	3.47e+01 & 	3.21e+02 & 	3.72e+01 & 	3.37e+01 & 	4.51e+00 & 	5.15e+00 & 	3.25e+01 & 	2.38e+02 & 	\textbf{1.64e+00} & 	2.93e+00 & 	2.89e+01 & 	3.48e+02 & 	2.28e+01 & 	3.24e+01 \\
% & $f_{34} (d=500)$ & 	1.89e+00 & 	2.10e+00 & 	2.10e+00 & 	4.12e+00 & 	3.75e-19 & 	1.05e+00 & 	1.49e+03 & 	3.08e+03 & 	3.15e+00 & 	\textbf{1.90e-22} & 	1.57e-13 & 	1.57e+00 & 	2.25e-14 & 	1.05e+00 \\
& {Wins \newline (MAD) } & \multicolumn{1}{c}{3} & \multicolumn{1}{c}{3} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{6} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{3} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{2} \\
%MTF.25OUT & MTF.LDO & CMAES.25OUT & CMAES.LDO & DE.25OUT & DE.LDO & PSO.X.25OUT & PSO.X.LDO & PSO.DE.25OUT & PSO.DE.LDO & DE.CMAES.25OUT & DE.CMAES.LDO & PSO.CMAES.25OUT & PSO.CMAES.LDO \\
\midrule
%Functions  1  -  7 \\
\multirow{2}{*}{\rotatebox[origin=c]{90}{SHU}} & Av.MAD  & \textbf{2.75e+02} & 1.61e+03 & 2.44e+03 & 2.09e+03 & 1.99e+04 & 5.56e+03 & 6.32e+02 & 6.92e+03 & 5.60e+02 & 6.41e+03 & 4.30e+03 & 1.99e+03 & 2.16e+03 & 2.42e+03 \\
& Av.Ranking  & \textbf{5.00} & 5.14 & 7.71 & 6.71 & 5.57 & 12.00 & 10.29 & 11.86 & 8.00 & 6.86 & 7.14 & 6.71 & 7.00 & 7.29 \\
\midrule
%Functions  8  -  11 \\
\multirow{2}{*}{\rotatebox[origin=c]{90}{MUL}} & Av.MAD  & 4.69e+02 & 5.79e+02 & 6.24e+02 & 4.96e+02 & 3.13e+02 & 4.10e+02 & 5.05e+03 & 1.20e+03 & 4.87e+02 & \textbf{9.82e+01} & 4.65e+02 & 4.42e+02 & 5.46e+02 & 4.87e+02 \\
& Av.Ranking  & 7.55 & 8.55 & 8.27 & 7.00 & 5.00 & 9.09 & 11.09 & 10.09 & 7.91 & \textbf{4.82} & 6.82 & 7.73 & 6.18 & 6.00 \\
\midrule
%Functions  12  -  19 \\
\multirow{2}{*}{\rotatebox[origin=c]{90}{HYB}} & Av.MAD  & 2.80e+02 & 3.96e+02 & 3.67e+02 & 3.02e+02 & 1.77e+02 & 4.13e+02 & 2.90e+03 & 7.75e+03 & 3.01e+02 & \textbf{6.69e+01} & 3.15e+02 & 2.90e+02 & 3.25e+02 & 2.86e+02 \\
& Av.Ranking  & \textbf{4.00} & 4.84 & 5.37 & 5.47 & 4.42 & 7.05 & 8.47 & 9.47 & 8.74 & 7.21 & 9.37 & 10.11 & 10.21 & 10.42 \\
\midrule
%Functions  1  -  19 \\
\multirow{2}{*}{\rotatebox[origin=c]{90}{ALL}} & Av.MAD  & \textbf{2.35e+02} & 7.88e+02 & 1.07e+03 & 9.13e+02 & 7.41e+03 & 2.33e+03 & 1.71e+03 & 6.44e+03 & 3.50e+02 & 2.40e+03 & 1.73e+03 & 8.81e+02 & 9.49e+02 & 1.03e+03 \\
& Av.Ranking  & 6.63 & 7.37 & 8.16 & 7.16 & \textbf{5.05} & 10.00 & 10.89 & 10.95 & 8.11 & 5.37 & 6.79 & 7.32 & 6.32 & 6.47 \\
\midrule
%Best algorithm across all functions: DE.25OUT	
%DE.25OUT 1 1 1 1 NA 1 0.36497709887089 1 1 1 1 1 1 1
& \multicolumn{1}{c}{Wilcoxon test} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} \\

    \end{longtable} }
\end{ThreePartTable}

==> tables/tbl_LD_2.tex <==
\begin{ThreePartTable}
\setlength{\tabcolsep}{0.5pt} % Default value: 6pt
    {\fontsize{6.5}{6.2}\selectfont
    \begin{longtable}{m{0.1cm} C{1.35cm} m{0.88cm} m{0.88cm} m{0.88cm} m{0.88cm} m{0.88cm} m{0.88cm} m{0.88cm} m{0.88cm} m{0.88cm} m{0.88cm} m{0.88cm} m{0.88cm} m{0.88cm} m{0.88cm}} %{@{} c | *{10}{c} @{}} %{ l c c c c c c c c c c c c c c c c}
    \caption{Average median (Av.MED), average median error (Av.MEDerr) and average median absolute deviation (Av.MAD) obtained by the algorithms on the 19 functions of the SOCO'10 test suite with with $\mathbf{d = 1\,000}$.}\label{table:MED-MEDerr-MAD-LD-1000}\\
    \toprule
    & $f\#$ &  
    %&  & 
    \textbf{\MTFtfoTBL} &  \textbf{\MTFldoTBL} & 
    \textbf{\CMAEStfoTBL} & \textbf{\CMAESldoTBL} & 
    \textbf{\DEtfoTBL} & \textbf{\DEldoTBL} & 
    \textbf{\PSOtfoTBL} & \textbf{\PSOldoTBL} & 
    \textbf{\PDHybtfoTBL} & \textbf{\PDHybldoTBL} & 
    \textbf{\DCHybtfoTBL} & \textbf{\DCHybldoTBL} &
    \textbf{\PCHybtfoTBL} & \textbf{\PCHybldoTBL} \\
    \midrule
    \endfirsthead
    
    \caption*{ Table \ref{table:MED-MEDerr-MAD-LD-1000} (Continued.)}\\
    \toprule
    & $f\#$ &  
    %&  & 
    \textbf{\MTFtfoTBL} &  \textbf{\MTFldoTBL} & 
    \textbf{\CMAEStfoTBL} & \textbf{\CMAESldoTBL} & 
    \textbf{\DEtfoTBL} & \textbf{\DEldoTBL} & 
    \textbf{\PSOtfoTBL} & \textbf{\PSOldoTBL} & 
    \textbf{\PDHybtfoTBL} & \textbf{\PDHybldoTBL} & 
    \textbf{\DCHybtfoTBL} & \textbf{\DCHybldoTBL} &
    \textbf{\PCHybtfoTBL} & \textbf{\PCHybldoTBL} \\
    \midrule
    \endhead
    
    \bottomrule
    %\insertTableNotes
    \endfoot
    
    \bottomrule
    %\insertTableNotes  % tell LaTeX where to insert the contents of "TableNotes"
    \endlastfoot

%%%%%%% Values here
%%%%% MED %%%%%
% \multirow{18}{*}{\rotatebox[origin=c]{90}{MEDIAN SOLUTION}} & $f_{1} (d=1000)$ & 	3.59e-21 & 	6.56e-20 & 	9.82e-17 & 	\textbf{2.47e-22} & 	3.24e-08 & 	1.24e+05 & 	7.63e+00 & 	2.86e+06 & 	8.21e-02 & 	1.06e-01 & 	2.25e-20 & 	2.74e-22 & 	8.66e-22 & 	1.02e-21 \\
% & $f_{5} (d=1000)$ & 	2.77e+01 & 	2.87e+01 & 	\textbf{1.67e+01} & 	2.62e+01 & 	1.60e+02 & 	1.50e+02 & 	1.12e+02 & 	1.16e+02 & 	1.33e+02 & 	1.67e+02 & 	2.68e+01 & 	3.23e+01 & 	3.10e+01 & 	2.19e+01 \\
% & $f_{6} (d=1000)$ & 	6.35e+05 & 	6.60e+05 & 	5.69e+05 & 	5.92e+05 & 	4.25e+06 & 	2.84e+06 & 	\textbf{4.25e+05} & 	3.25e+06 & 	1.61e+06 & 	4.04e+06 & 	7.46e+05 & 	7.87e+05 & 	7.96e+05 & 	6.30e+05 \\
% & $f_{8} (d=1000)$ & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 & 	\textbf{2.75e-04} & 	3.37e+02 & 	2.80e+03 & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 \\
% & $f_{9} (d=1000)$ & 	8.17e+01 & 	4.29e+01 & 	3.73e+01 & 	1.85e+02 & 	9.07e+02 & 	5.42e+03 & 	6.94e+03 & 	9.20e+03 & 	2.94e+03 & 	1.48e+03 & 	4.88e+00 & 	6.49e+01 & 	\textbf{4.23e+00} & 	1.36e+01 \\
% & $f_{10} (d=1000)$ & 	1.76e+01 & 	1.36e+01 & 	4.14e+01 & 	2.62e+01 & 	\textbf{2.08e-03} & 	5.36e+03 & 	7.96e+02 & 	6.17e+04 & 	4.24e+01 & 	6.01e-01 & 	8.11e+00 & 	1.13e+01 & 	6.71e+00 & 	1.78e+01 \\
% & $f_{13} (d=1000)$ & 	5.77e-13 & 	2.59e-12 & 	\textbf{3.29e-13} & 	4.97e-13 & 	6.42e-03 & 	1.66e+01 & 	1.95e+01 & 	2.11e+01 & 	3.65e-01 & 	1.31e-01 & 	8.38e-13 & 	6.00e-13 & 	8.68e-13 & 	6.72e-13 \\
% & $f_{15} (d=1000)$ & 	9.68e+02 & 	9.69e+02 & 	9.73e+02 & 	\textbf{9.67e+02} & 	3.18e+03 & 	1.00e+10 & 	2.39e+05 & 	1.00e+10 & 	1.21e+04 & 	5.04e+03 & 	9.75e+02 & 	9.74e+02 & 	9.76e+02 & 	9.72e+02 \\
% & $f_{17} (d=1000)$ & 	3.25e-19 & 	4.61e-19 & 	1.26e-16 & 	4.34e-19 & 	2.45e-05 & 	1.99e+03 & 	1.51e+00 & 	2.60e+04 & 	1.80e-01 & 	1.05e-02 & 	\textbf{2.71e-19} & 	4.34e-19 & 	\textbf{2.71e-19} & 	3.25e-19 \\
% & $f_{19} (d=1000)$ & 	8.38e+02 & 	7.86e+02 & 	1.17e+03 & 	9.85e+02 & 	1.14e+03 & 	3.35e+04 & 	5.11e+04 & 	2.95e+05 & 	4.87e+03 & 	1.72e+03 & 	7.00e+02 & 	1.24e+03 & 	\textbf{6.50e+02} & 	9.18e+02 \\
% & $f_{21} (d=1000)$ & 	5.22e+05 & 	5.17e+05 & 	5.26e+05 & 	5.34e+05 & 	\textbf{4.59e+05} & 	6.07e+05 & 	7.05e+05 & 	7.83e+05 & 	5.79e+05 & 	4.77e+05 & 	5.00e+05 & 	5.22e+05 & 	4.99e+05 & 	5.08e+05 \\
% & $f_{27} (d=1000)$ & 	1.80e+03 & 	1.74e+03 & 	1.79e+03 & 	1.88e+03 & 	\textbf{3.36e+01} & 	1.27e+05 & 	2.29e+03 & 	2.04e+06 & 	8.18e+02 & 	1.25e+02 & 	1.53e+03 & 	1.75e+03 & 	1.47e+03 & 	1.67e+03 \\
% & $f_{28} (d=1000)$ & 	2.62e+03 & 	2.56e+03 & 	2.64e+03 & 	2.71e+03 & 	3.56e+03 & 	1.00e+10 & 	1.04e+04 & 	1.00e+10 & 	1.28e+04 & 	6.40e+03 & 	2.40e+03 & 	2.58e+03 & 	\textbf{2.37e+03} & 	2.53e+03 \\
% & $f_{29} (d=1000)$ & 	1.28e+03 & 	1.14e+03 & 	1.17e+03 & 	1.45e+03 & 	\textbf{4.47e+02} & 	4.68e+03 & 	7.48e+03 & 	1.34e+04 & 	2.58e+03 & 	4.80e+02 & 	8.46e+02 & 	1.20e+03 & 	8.13e+02 & 	1.01e+03 \\
% & $f_{30} (d=1000)$ & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 & 	\textbf{2.14e-03} & 	1.41e+03 & 	1.38e+04 & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 \\
% & $f_{31} (d=1000)$ & 	3.56e+03 & 	3.41e+03 & 	3.51e+03 & 	3.74e+03 & 	\textbf{1.94e+02} & 	8.04e+04 & 	4.55e+03 & 	1.15e+06 & 	1.91e+03 & 	4.79e+02 & 	2.89e+03 & 	3.46e+03 & 	2.71e+03 & 	3.26e+03 \\
% & $f_{32} (d=1000)$ & 	6.10e+03 & 	5.94e+03 & 	6.22e+03 & 	6.32e+03 & 	\textbf{1.87e+03} & 	1.66e+09 & 	8.17e+03 & 	6.12e+08 & 	4.12e+03 & 	2.94e+03 & 	5.39e+03 & 	5.99e+03 & 	5.21e+03 & 	5.82e+03 \\
% & $f_{33} (d=1000)$ & 	1.18e+03 & 	1.06e+03 & 	1.09e+03 & 	1.30e+03 & 	\textbf{1.89e+02} & 	1.81e+03 & 	3.37e+03 & 	3.65e+03 & 	1.23e+03 & 	2.61e+02 & 	6.63e+02 & 	1.13e+03 & 	5.70e+02 & 	9.29e+02 \\
% & $f_{34} (d=1000)$ & 	2.73e+01 & 	1.68e+01 & 	1.75e+01 & 	4.32e+01 & 	2.10e+00 & 	2.69e+03 & 	3.69e+04 & 	5.55e+04 & 	3.52e+01 & 	\textbf{6.63e-02} & 	2.10e+00 & 	2.33e+01 & 	1.78e+00 & 	8.40e+00 \\
& {Wins \newline (MED) } & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{9} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{4} & \multicolumn{1}{c}{0} \\
%MTF.25OUT & MTF.LDO & CMAES.25OUT & CMAES.LDO & DE.25OUT & DE.LDO & PSO.X.25OUT & PSO.X.LDO & PSO.DE.25OUT & PSO.DE.LDO & DE.CMAES.25OUT & DE.CMAES.LDO & PSO.CMAES.25OUT & PSO.CMAES.LDO \\
\midrule
%Functions  1  -  7 \\
\multirow{2}{*}{\rotatebox[origin=c]{90}{SHU}} & Av.MED  & 1.43e+09 & 1.43e+09 & 1.43e+09 & 1.43e+09 & 6.07e+05 & 4.25e+05 & \textbf{6.22e+04} & 1.43e+09 & 1.43e+09 & 1.43e+09 & 1.43e+09 & 1.43e+09 & 1.43e+09 & 1.43e+09 \\
& Av.Ranking  & 6.57 & 7.43 & \textbf{5.71} & \textbf{5.71} & 8.00 & 10.71 & 9.00 & 13.14 & 11.14 & 10.57 & 6.14 & 6.71 & 6.29 & \textbf{5.71} \\
\midrule
%Functions  8  -  11 \\
\multirow{2}{*}{\rotatebox[origin=c]{90}{MUL}} & Av.MED  & 1.05e+05 & 1.04e+05 & 1.06e+05 & 1.07e+05 & \textbf{9.27e+04} & 2.00e+09 & 1.99e+05 & 2.00e+09 & 1.19e+05 & 9.68e+04 & 1.00e+05 & 1.05e+05 & 1.00e+05 & 1.02e+05 \\
& Av.Ranking  & 7.73 & 6.36 & 8.45 & 9.00 & \textbf{3.73} & 11.91 & 11.45 & 13.91 & 9.09 & 6.00 & 4.91 & 8.00 & 4.27 & 5.73 \\
\midrule
%Functions  12  -  19 \\
\multirow{2}{*}{\rotatebox[origin=c]{90}{HYB}} & Av.MED  & 1.11e+09 & 1.11e+09 & 1.11e+09 & 1.11e+09 & \textbf{5.17e+04} & 1.30e+09 & 8.80e+04 & 2.29e+09 & 1.11e+09 & 1.11e+09 & 1.11e+09 & 1.11e+09 & 1.11e+09 & 1.11e+09 \\
& Av.Ranking  & 4.58 & 4.16 & 5.42 & 6.89 & \textbf{3.89} & 8.32 & 8.74 & 10.47 & 8.68 & 7.63 & 8.63 & 10.47 & 9.37 & 10.74 \\
\midrule
%Functions  1  -  19 \\
\multirow{2}{*}{\rotatebox[origin=c]{90}{ALL}} & Av.MED  & 1.05e+09 & 1.05e+09 & 1.05e+09 & 1.05e+09 & 2.48e+05 & 1.14e+09 & \textbf{7.99e+04} & 2.14e+09 & 1.05e+09 & 1.05e+09 & 1.05e+09 & 1.05e+09 & 1.05e+09 & 1.05e+09 \\
& Av.Ranking  & 7.37 & 6.74 & 7.37 & 7.89 & 5.32 & 11.47 & 10.63 & 13.63 & 9.89 & 7.42 & 5.32 & 7.53 & \textbf{4.89} & 5.68 \\
\midrule
%Best algorithm across all functions: PSO.CMAES.25OUT	
%PSO.CMAES.25OUT 1 1 1 1 1 1 1 0.0292154044626484 1 1 1 1 NA 1
& \multicolumn{1}{c}{Wilcoxon test} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$+$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\approx$} \\

%%%%% MEDerr %%%%%
\toprule
% \multirow{18}{*}{\rotatebox[origin=c]{90}{MEDIAN SOLUTION ERROR}} & $f_{1} (d=1000)$ & 	3.37e-21 & 	6.54e-20 & 	9.82e-17 & 	\textbf{2.51e-23} & 	3.24e-08 & 	1.24e+05 & 	7.63e+00 & 	2.86e+06 & 	8.21e-02 & 	1.06e-01 & 	2.23e-20 & 	5.21e-23 & 	6.44e-22 & 	7.98e-22 \\
% & $f_{5} (d=1000)$ & 	1.36e+01 & 	1.46e+01 & 	\textbf{2.61e+00} & 	1.21e+01 & 	1.46e+02 & 	1.36e+02 & 	9.79e+01 & 	1.02e+02 & 	1.19e+02 & 	1.53e+02 & 	1.27e+01 & 	1.82e+01 & 	1.69e+01 & 	7.81e+00 \\
% & $f_{6} (d=1000)$ & 	3.47e+05 & 	3.72e+05 & 	2.81e+05 & 	3.04e+05 & 	3.96e+06 & 	2.55e+06 & 	\textbf{1.37e+05} & 	2.96e+06 & 	1.32e+06 & 	3.75e+06 & 	4.58e+05 & 	4.99e+05 & 	5.08e+05 & 	3.42e+05 \\
% & $f_{8} (d=1000)$ & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 & 	\textbf{4.68e-05} & 	3.37e+02 & 	2.80e+03 & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 \\
% & $f_{9} (d=1000)$ & 	7.82e+01 & 	3.94e+01 & 	3.38e+01 & 	1.81e+02 & 	9.03e+02 & 	5.42e+03 & 	6.94e+03 & 	9.20e+03 & 	2.94e+03 & 	1.48e+03 & 	1.35e+00 & 	6.14e+01 & 	\textbf{7.03e-01} & 	1.01e+01 \\
% & $f_{10} (d=1000)$ & 	1.76e+01 & 	1.36e+01 & 	4.14e+01 & 	2.62e+01 & 	\textbf{2.06e-03} & 	5.36e+03 & 	7.96e+02 & 	6.17e+04 & 	4.24e+01 & 	6.01e-01 & 	8.11e+00 & 	1.13e+01 & 	6.71e+00 & 	1.78e+01 \\
% & $f_{13} (d=1000)$ & 	2.59e-13 & 	2.27e-12 & 	\textbf{1.12e-14} & 	1.79e-13 & 	6.42e-03 & 	1.66e+01 & 	1.95e+01 & 	2.11e+01 & 	3.65e-01 & 	1.31e-01 & 	5.20e-13 & 	2.82e-13 & 	5.50e-13 & 	3.54e-13 \\
% & $f_{15} (d=1000)$ & 	3.20e+00 & 	4.20e+00 & 	8.20e+00 & 	\textbf{2.20e+00} & 	2.22e+03 & 	1.00e+10 & 	2.38e+05 & 	1.00e+10 & 	1.11e+04 & 	4.08e+03 & 	1.02e+01 & 	9.20e+00 & 	1.12e+01 & 	7.20e+00 \\
% & $f_{17} (d=1000)$ & 	1.08e-19 & 	2.44e-19 & 	1.26e-16 & 	2.17e-19 & 	2.45e-05 & 	1.99e+03 & 	1.51e+00 & 	2.60e+04 & 	1.80e-01 & 	1.05e-02 & 	\textbf{5.42e-20} & 	2.17e-19 & 	\textbf{5.42e-20} & 	1.08e-19 \\
% & $f_{19} (d=1000)$ & 	2.41e+02 & 	1.89e+02 & 	5.73e+02 & 	3.88e+02 & 	5.43e+02 & 	3.29e+04 & 	5.05e+04 & 	2.94e+05 & 	4.27e+03 & 	1.12e+03 & 	1.03e+02 & 	6.43e+02 & 	\textbf{5.30e+01} & 	3.21e+02 \\
% & $f_{21} (d=1000)$ & 	7.41e+04 & 	6.91e+04 & 	7.81e+04 & 	8.61e+04 & 	\textbf{1.11e+04} & 	1.59e+05 & 	2.57e+05 & 	3.35e+05 & 	1.31e+05 & 	2.91e+04 & 	5.21e+04 & 	7.41e+04 & 	5.11e+04 & 	6.01e+04 \\
% & $f_{27} (d=1000)$ & 	1.79e+03 & 	1.73e+03 & 	1.78e+03 & 	1.87e+03 & 	\textbf{2.23e+01} & 	1.27e+05 & 	2.28e+03 & 	2.04e+06 & 	8.07e+02 & 	1.14e+02 & 	1.52e+03 & 	1.74e+03 & 	1.46e+03 & 	1.66e+03 \\
% & $f_{28} (d=1000)$ & 	4.36e+02 & 	3.76e+02 & 	4.56e+02 & 	5.26e+02 & 	1.38e+03 & 	1.00e+10 & 	8.22e+03 & 	1.00e+10 & 	1.06e+04 & 	4.22e+03 & 	2.16e+02 & 	3.96e+02 & 	\textbf{1.86e+02} & 	3.46e+02 \\
% & $f_{29} (d=1000)$ & 	1.06e+03 & 	9.17e+02 & 	9.47e+02 & 	1.23e+03 & 	\textbf{2.24e+02} & 	4.46e+03 & 	7.26e+03 & 	1.32e+04 & 	2.36e+03 & 	2.57e+02 & 	6.23e+02 & 	9.77e+02 & 	5.90e+02 & 	7.87e+02 \\
% & $f_{30} (d=1000)$ & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 & 	\textbf{2.06e-03} & 	1.41e+03 & 	1.38e+04 & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 & 	1.00e+10 \\
% & $f_{31} (d=1000)$ & 	3.47e+03 & 	3.32e+03 & 	3.42e+03 & 	3.65e+03 & 	\textbf{1.06e+02} & 	8.03e+04 & 	4.46e+03 & 	1.15e+06 & 	1.82e+03 & 	3.91e+02 & 	2.80e+03 & 	3.37e+03 & 	2.62e+03 & 	3.17e+03 \\
% & $f_{32} (d=1000)$ & 	4.83e+03 & 	4.67e+03 & 	4.95e+03 & 	5.05e+03 & 	\textbf{6.03e+02} & 	1.66e+09 & 	6.90e+03 & 	6.12e+08 & 	2.85e+03 & 	1.67e+03 & 	4.12e+03 & 	4.72e+03 & 	3.94e+03 & 	4.55e+03 \\
% & $f_{33} (d=1000)$ & 	1.05e+03 & 	9.28e+02 & 	9.58e+02 & 	1.17e+03 & 	\textbf{5.73e+01} & 	1.68e+03 & 	3.24e+03 & 	3.52e+03 & 	1.10e+03 & 	1.29e+02 & 	5.31e+02 & 	9.98e+02 & 	4.38e+02 & 	7.97e+02 \\
% & $f_{34} (d=1000)$ & 	2.73e+01 & 	1.68e+01 & 	1.75e+01 & 	4.32e+01 & 	2.10e+00 & 	2.69e+03 & 	3.69e+04 & 	5.55e+04 & 	3.52e+01 & 	\textbf{6.63e-02} & 	2.10e+00 & 	2.33e+01 & 	1.78e+00 & 	8.40e+00 \\
& {Wins \newline (MEDerr) } & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{9} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{4} & \multicolumn{1}{c}{0} \\
%MTF.25OUT & MTF.LDO & CMAES.25OUT & CMAES.LDO & DE.25OUT & DE.LDO & PSO.X.25OUT & PSO.X.LDO & PSO.DE.25OUT & PSO.DE.LDO & DE.CMAES.25OUT & DE.CMAES.LDO & PSO.CMAES.25OUT & PSO.CMAES.LDO \\
\midrule
%Functions  1  -  7 \\
\multirow{2}{*}{\rotatebox[origin=c]{90}{SHU}} & Av.MEDerr  & 1.43e+09 & 1.43e+09 & 1.43e+09 & 1.43e+09 & 5.66e+05 & 3.84e+05 & \textbf{2.11e+04} & 1.43e+09 & 1.43e+09 & 1.43e+09 & 1.43e+09 & 1.43e+09 & 1.43e+09 & 1.43e+09 \\
& Av.Ranking  & 6.57 & 7.43 & \textbf{5.71} & \textbf{5.71} & 8.00 & 10.71 & 9.00 & 13.14 & 11.14 & 10.57 & 6.14 & 6.71 & 6.29 & \textbf{5.71} \\
\midrule
%Functions  8  -  11 \\
\multirow{2}{*}{\rotatebox[origin=c]{90}{MUL}} & Av.MEDerr  & 1.49e+04 & 1.39e+04 & 1.57e+04 & 1.73e+04 & \textbf{2.77e+03} & 2.00e+09 & 1.09e+05 & 2.00e+09 & 2.93e+04 & 6.86e+03 & 1.04e+04 & 1.50e+04 & 1.02e+04 & 1.21e+04 \\
& Av.Ranking  & 7.73 & 6.36 & 8.45 & 9.00 & \textbf{3.73} & 11.91 & 11.45 & 13.91 & 9.09 & 6.00 & 4.91 & 8.00 & 4.27 & 5.73 \\
\midrule
%Functions  12  -  19 \\
\multirow{2}{*}{\rotatebox[origin=c]{90}{HYB}} & Av.MEDerr  & 1.11e+09 & 1.11e+09 & 1.11e+09 & 1.11e+09 & \textbf{1.50e+03} & 1.30e+09 & 3.78e+04 & 2.29e+09 & 1.11e+09 & 1.11e+09 & 1.11e+09 & 1.11e+09 & 1.11e+09 & 1.11e+09 \\
& Av.Ranking  & 4.58 & 4.16 & 5.42 & 6.89 & \textbf{3.89} & 8.32 & 8.74 & 10.47 & 8.68 & 7.63 & 8.63 & 10.47 & 9.37 & 10.74 \\
\midrule
%Functions  1  -  19 \\
\multirow{2}{*}{\rotatebox[origin=c]{90}{ALL}} & Av.MEDerr  & 1.05e+09 & 1.05e+09 & 1.05e+09 & 1.05e+09 & 2.09e+05 & 1.14e+09 & \textbf{4.09e+04} & 2.14e+09 & 1.05e+09 & 1.05e+09 & 1.05e+09 & 1.05e+09 & 1.05e+09 & 1.05e+09 \\
& Av.Ranking  & 7.37 & 6.74 & 7.37 & 7.89 & 5.32 & 11.47 & 10.63 & 13.63 & 9.89 & 7.42 & 5.32 & 7.53 & \textbf{4.89} & 5.68 \\
\midrule
%Best algorithm across all functions: PSO.CMAES.25OUT	
%PSO.CMAES.25OUT 1 1 1 1 1 1 1 0.0292154044626484 1 1 1 1 NA 1
& \multicolumn{1}{c}{Wilcoxon test} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$+$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\approx$} \\

%%%%% MAD %%%%%
\toprule
% \multirow{18}{*}{\rotatebox[origin=c]{90}{MEDIAN ABSOLUTE DEVIATION}} & $f_{1} (d=1000)$ & 	1.31e-22 & 	3.22e-23 & 	3.08e-18 & 	1.76e-23 & 	9.42e-02 & 	2.00e+03 & 	1.66e+01 & 	1.45e+05 & 	3.73e-02 & 	1.05e-02 & 	1.40e-21 & 	\textbf{1.50e-23} & 	1.53e-23 & 	4.47e-23 \\
% & $f_{5} (d=1000)$ & 	2.26e+00 & 	2.77e+00 & 	2.14e+00 & 	1.61e+00 & 	2.53e+00 & 	3.27e+00 & 	\textbf{1.52e+00} & 	4.57e+00 & 	3.73e+00 & 	2.64e+00 & 	1.79e+00 & 	3.46e+00 & 	2.74e+00 & 	2.66e+00 \\
% & $f_{6} (d=1000)$ & 	3.22e+04 & 	2.88e+04 & 	\textbf{1.58e+03} & 	1.70e+04 & 	3.71e+05 & 	3.28e+05 & 	1.77e+05 & 	3.13e+05 & 	2.69e+04 & 	1.73e+05 & 	1.95e+04 & 	1.86e+04 & 	4.19e+04 & 	2.57e+04 \\
% & $f_{8} (d=1000)$ & 	\textbf{0.00e+00} & 	\textbf{0.00e+00} & 	\textbf{0.00e+00} & 	\textbf{0.00e+00} & 	3.26e-05 & 	3.46e+00 & 	1.85e+01 & 	\textbf{0.00e+00} & 	\textbf{0.00e+00} & 	\textbf{0.00e+00} & 	\textbf{0.00e+00} & 	\textbf{0.00e+00} & 	\textbf{0.00e+00} & 	\textbf{0.00e+00} \\
% & $f_{9} (d=1000)$ & 	2.46e+00 & 	2.78e+00 & 	1.03e+01 & 	3.34e+01 & 	1.40e+01 & 	3.77e+01 & 	1.27e+02 & 	1.01e+02 & 	1.58e+02 & 	3.14e+01 & 	1.38e+00 & 	2.79e+01 & 	\textbf{3.62e-01} & 	2.21e+00 \\
% & $f_{10} (d=1000)$ & 	3.44e+00 & 	4.60e-01 & 	4.58e-01 & 	4.24e+00 & 	\textbf{2.81e-04} & 	1.73e+02 & 	2.37e+01 & 	3.06e+03 & 	1.94e+01 & 	3.71e-02 & 	1.57e+00 & 	3.44e+00 & 	3.79e+00 & 	2.35e+00 \\
% & $f_{13} (d=1000)$ & 	2.63e-14 & 	2.75e-13 & 	2.58e-15 & 	\textbf{1.99e-15} & 	1.26e-01 & 	2.28e-01 & 	1.67e-02 & 	3.68e-02 & 	3.72e-02 & 	1.59e-01 & 	2.26e-14 & 	3.17e-15 & 	1.43e-14 & 	1.62e-14 \\
% & $f_{15} (d=1000)$ & 	2.06e-01 & 	3.02e-01 & 	2.18e-01 & 	1.80e-01 & 	2.98e+02 & 	\textbf{0.00e+00} & 	2.40e+05 & 	\textbf{0.00e+00} & 	3.22e+03 & 	3.08e+02 & 	3.27e-01 & 	2.24e-01 & 	2.96e-01 & 	3.17e-01 \\
% & $f_{17} (d=1000)$ & 	2.61e-22 & 	2.73e-20 & 	3.28e-18 & 	5.39e-20 & 	1.68e-05 & 	3.40e+01 & 	1.79e+00 & 	1.55e+03 & 	2.15e-01 & 	2.74e-03 & 	\textbf{5.05e-23} & 	3.19e-22 & 	\textbf{5.05e-23} & 	2.61e-22 \\
% & $f_{19} (d=1000)$ & 	2.98e+01 & 	3.38e+01 & 	3.44e+01 & 	4.38e+01 & 	1.03e+02 & 	2.62e+03 & 	5.35e+03 & 	3.28e+04 & 	2.38e+02 & 	\textbf{1.67e+01} & 	3.13e+01 & 	3.98e+01 & 	2.91e+01 & 	4.89e+01 \\
% & $f_{21} (d=1000)$ & 	3.85e+03 & 	4.51e+03 & 	2.93e+03 & 	\textbf{1.97e+02} & 	1.77e+03 & 	1.38e+04 & 	6.08e+04 & 	1.81e+03 & 	3.88e+03 & 	1.60e+03 & 	3.23e+03 & 	3.49e+03 & 	3.26e+03 & 	3.86e+03 \\
% & $f_{27} (d=1000)$ & 	1.80e+01 & 	1.87e+01 & 	2.71e+01 & 	3.45e+01 & 	\textbf{2.42e+00} & 	3.35e+03 & 	4.48e+01 & 	2.72e+05 & 	1.73e+02 & 	3.46e+00 & 	3.79e+01 & 	3.85e+01 & 	4.15e+01 & 	2.21e+01 \\
% & $f_{28} (d=1000)$ & 	4.09e+01 & 	2.33e+01 & 	3.53e+01 & 	3.88e+01 & 	3.00e+02 & 	\textbf{0.00e+00} & 	1.13e+04 & 	\textbf{0.00e+00} & 	2.90e+03 & 	2.81e+02 & 	3.46e+01 & 	1.76e+01 & 	3.60e+01 & 	3.20e+01 \\
% & $f_{29} (d=1000)$ & 	2.48e+01 & 	4.04e+01 & 	2.75e+01 & 	3.00e+01 & 	3.00e+01 & 	3.78e+01 & 	3.76e+02 & 	3.31e+02 & 	1.87e+01 & 	2.28e+01 & 	\textbf{1.62e+01} & 	3.76e+01 & 	1.70e+01 & 	3.13e+01 \\
% & $f_{30} (d=1000)$ & 	\textbf{0.00e+00} & 	\textbf{0.00e+00} & 	\textbf{0.00e+00} & 	\textbf{0.00e+00} & 	2.24e-04 & 	3.63e+01 & 	2.97e+03 & 	\textbf{0.00e+00} & 	\textbf{0.00e+00} & 	\textbf{0.00e+00} & 	\textbf{0.00e+00} & 	\textbf{0.00e+00} & 	\textbf{0.00e+00} & 	\textbf{0.00e+00} \\
% & $f_{31} (d=1000)$ & 	3.02e+01 & 	3.59e+01 & 	2.47e+01 & 	4.18e+01 & 	1.64e+01 & 	2.09e+04 & 	\textbf{1.38e+01} & 	2.43e+04 & 	2.59e+02 & 	1.98e+02 & 	4.03e+01 & 	2.30e+01 & 	1.18e+02 & 	4.42e+01 \\
% & $f_{32} (d=1000)$ & 	4.30e+01 & 	\textbf{1.80e+01} & 	2.45e+01 & 	4.16e+01 & 	2.70e+02 & 	4.46e+09 & 	2.94e+02 & 	2.05e+08 & 	3.99e+02 & 	1.11e+02 & 	4.57e+01 & 	2.70e+01 & 	3.32e+01 & 	1.90e+01 \\
% & $f_{33} (d=1000)$ & 	3.19e+01 & 	2.85e+01 & 	4.68e+01 & 	3.75e+01 & 	1.88e+01 & 	2.00e+02 & 	1.32e+02 & 	1.99e+02 & 	1.85e+01 & 	\textbf{3.03e+00} & 	3.60e+01 & 	3.83e+01 & 	2.26e+01 & 	2.05e+01 \\
% & $f_{34} (d=1000)$ & 	4.19e+00 & 	2.10e+00 & 	3.46e-01 & 	5.04e+00 & 	1.05e+00 & 	2.85e+02 & 	1.97e+03 & 	4.13e+03 & 	3.09e+00 & 	\textbf{5.36e-03} & 	1.89e+00 & 	4.20e+00 & 	3.20e-01 & 	2.62e+00 \\
& {Wins \newline (MAD) } & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3} & \multicolumn{1}{c}{3} & \multicolumn{1}{c}{4} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{4} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{5} & \multicolumn{1}{c}{4} & \multicolumn{1}{c}{3} & \multicolumn{1}{c}{4} & \multicolumn{1}{c}{2} \\
%MTF.25OUT & MTF.LDO & CMAES.25OUT & CMAES.LDO & DE.25OUT & DE.LDO & PSO.X.25OUT & PSO.X.LDO & PSO.DE.25OUT & PSO.DE.LDO & DE.CMAES.25OUT & DE.CMAES.LDO & PSO.CMAES.25OUT & PSO.CMAES.LDO \\
\midrule
%Functions  1  -  7 \\
\multirow{2}{*}{\rotatebox[origin=c]{90}{SHU}} & Av.MAD  & 4.60e+03 & 4.12e+03 & \textbf{2.28e+02} & 2.43e+03 & 5.30e+04 & 4.72e+04 & 2.53e+04 & 6.59e+04 & 3.87e+03 & 2.47e+04 & 2.79e+03 & 2.66e+03 & 5.99e+03 & 3.67e+03 \\
& Av.Ranking  & 7.00 & 7.00 & \textbf{5.00} & 5.57 & 9.00 & 12.57 & 10.29 & 12.43 & 10.86 & 8.71 & 5.43 & 6.57 & 6.43 & 6.14 \\
\midrule
%Functions  8  -  11 \\
\multirow{2}{*}{\rotatebox[origin=c]{90}{MUL}} & Av.MAD  & 7.76e+02 & 9.09e+02 & 5.93e+02 & \textbf{4.82e+01} & 4.34e+02 & 3.29e+03 & 6.12e+04 & 7.23e+03 & 1.47e+03 & 3.85e+02 & 6.52e+02 & 7.06e+02 & 6.58e+02 & 7.82e+02 \\
& Av.Ranking  & \textbf{6.18} & 6.82 & 6.55 & 7.00 & 7.36 & 10.91 & 11.82 & 10.36 & 10.09 & 6.73 & 6.45 & 6.91 & 6.27 & 7.00 \\
\midrule
%Functions  12  -  19 \\
\multirow{2}{*}{\rotatebox[origin=c]{90}{HYB}} & Av.MAD  & 4.49e+02 & 5.20e+02 & 3.46e+02 & \textbf{4.74e+01} & 2.68e+02 & 4.96e+08 & 8.66e+03 & 2.28e+07 & 8.50e+02 & 2.47e+02 & 3.83e+02 & 4.08e+02 & 3.92e+02 & 4.48e+02 \\
& Av.Ranking  & \textbf{3.58} & 3.79 & 4.42 & 5.95 & 5.63 & 8.32 & 8.79 & 9.58 & 9.05 & 8.42 & 9.21 & 10.11 & 10.32 & 10.84 \\
\midrule
%Functions  1  -  19 \\
\multirow{2}{*}{\rotatebox[origin=c]{90}{ALL}} & Av.MAD  & 1.91e+03 & 1.76e+03 & \textbf{2.50e+02} & 9.22e+02 & 1.97e+04 & 2.35e+08 & 2.63e+04 & 1.08e+07 & 2.01e+03 & 9.24e+03 & 1.21e+03 & 1.18e+03 & 2.39e+03 & 1.57e+03 \\
& Av.Ranking  & 6.63 & 6.84 & \textbf{5.79} & 6.68 & 7.79 & 11.58 & 11.32 & 11.32 & 10.26 & 7.16 & 6.00 & 6.95 & 6.11 & 6.68 \\
\midrule
%Best algorithm across all functions: CMAES.25OUT	
%CMAES.25OUT 1 1 NA 1 1 0.0527979649976668 0.033564085589459 0.303564959476053 0.303564959476053 1 1 1 1 1
& \multicolumn{1}{c}{Wilcoxon test} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$+$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} & \multicolumn{1}{c}{$\approx$} \\
    \end{longtable} }
\end{ThreePartTable}
